AC3D: Analyzing and Improving 3D Camera Control in Video Diffusion Transformers

Numerous works have recently integrated 3D camera control into foundational text-to-video models, but the resulting camera control is often imprecise, and video generation quality suffers. In this work, we analyze camera motion from a first principles perspective, uncovering insights that enable precise 3D camera manipulation without compromising synthesis quality. First, we determine that motion induced by camera movements in videos is low-frequency in nature. This motivates us to adjust train and test pose conditioning schedules, accelerating training convergence while improving visual and motion quality. Then, by probing the representations of an unconditional video diffusion transformer, we observe that they implicitly perform camera pose estimation under the hood, and only a sub-portion of their layers contain the camera information. This suggested us to limit the injection of camera conditioning to a subset of the architecture to prevent interference with other video features, leading to a 4x reduction of training parameters, improved training speed, and 10% higher visual quality. Finally, we complement the typical dataset for camera control learning with a curated dataset of 20K diverse, dynamic videos with stationary cameras. This helps the model distinguish between camera and scene motion and improves the dynamics of generated pose-conditioned videos. We compound these findings to design the Advanced 3D Camera Control (AC3D) architecture, the new state-of-the-art model for generative video modeling with camera control.

==> figures/camera-motion-analysis-old.tex <==
\newcommand{\motionlfigw}{0.25\linewidth}
\newcommand{\motionlfigh}{3.1cm}
\newcommand{\motionmidfigw}{0.3\linewidth}
\newcommand{\motionrfigw}{0.45\linewidth}

\begin{figure*}
\centering
\begin{subfigure}[t]{\motionlfigw}
\vspace{0.05cm}
\includegraphics[width=\linewidth,height=\motionlfigh]{images/video-cropped.pdf}
\caption{A generated video at different denoising steps. The camera has already been decided by the model even at $t = 0.9$ (first 10\% of the recflow reverse process) and does not change since then. \gqc{text resolution at left is very low resolution.}}
\end{subfigure}%
\hfill
\begin{subfigure}[t]{\motionmidfigw}
\vspace{0pt}
\includegraphics[width=\linewidth]{images/ampl.pdf}
\end{subfigure}%
\hfill
\begin{subfigure}[t]{\motionrfigw}
\vspace{0pt}
\includegraphics[width=\linewidth]{images/ampl-ratio.pdf}
\end{subfigure}%
\caption{
\textbf{How camera motion is modeled by video diffusion.}
We observe that the motion induced by camera transitions is a low-frequency type of motion and is created by a video diffusion model during the first ${\approx}$20\% of the denoising process. \gqc{does not align with what said in fig (a), 10\%.}
\sout{This is also confirmed by our visualizations in \todo{where?} and the supp.}\gq{as visualized in (a).}
Controlling the camera later in the denoising trajectory is not only unnecessary but \emph{detrimental} to both scene motion and overall visual quality (demonstrated by our experiments in \cref{sec:experiments} show). \gqc{lacks analysis of the spectrum, correlation between motion and camera}
}
\label{fig:camera-motion-analysis}
\end{figure*}

==> figures/comparisons.tex <==
\begin{figure*}
\centering
\includegraphics[width=6.9in, height=1in]{example-image-a}
\captionof{figure}{\textbf{Qualitative evaluation.}
\AT{I'd STRONGLY suggest to not have images for comparisons, but instead suggest the reader to go to the supplementary material DIRECTLY.
Video frames on papers.... are useless.}
}
\label{fig:comparisons}
\end{figure*}

==> figures/data-analysis.tex <==
\begin{figure*}
\centering
\includegraphics[width=\textwidth,height=5cm]{example-image-a}
\caption{We found missing mode in the modern 3d camera datasets. In practice, it turned out to be easy to fill. Modern datasets used by 3D camera control papers rely exlusively on videos. We found that the gap can be closed with an easy-to-collect dataset of in-the-wild videos with static camera and scene motion.}
\label{fig:data-analysis}
\end{figure*}


==> figures/linprob-analysis-old.tex <==
\newcommand{\linprobfigwidth}{0.49\linewidth}

\begin{figure}
\centering
\begin{subfigure}[t]{\linprobfigwidth}
\vspace{0.05cm}
\includegraphics[width=\linewidth]{images/rotation-r2.pdf}
\caption{Rotation R2 score on the test set.}
\end{subfigure}%
\hfill
\begin{subfigure}[t]{\linprobfigwidth}
\vspace{0pt}
\includegraphics[width=\linewidth]{images/translation-r2.pdf}
\caption{Rotation R2 score on the test set.}
\end{subfigure}%
\caption{\textbf{Which blocks model the camera motion in video diffusion transformers?} We perform linear probing of camera parameters (rotation and translation) in each of our video DiT block for various noise levels and observe that later blocks carry more knowledge about the camera while the earlier ones contain little of it. This indicates that the camera should be modeled in the early blocks to allow the later ones to produce the features that are aligned with the global camera motion.
\gqc{My immediate thought is: why not directly injected into the last block.}
}
\label{fig:linprob-analysis}
\end{figure}


==> rebuttal/fig/analysis.tex <==
\centering
%\includegraphics[width=0.25\textwidth, height=3cm]{example-image-a}
\includegraphics[width=0.2\textwidth, height=1.9cm]{rebuttal/imgs/ampl-per-cam.pdf}
%\includegraphics[width=0.23\textwidth, height=3cm]{example-image-a}
\hspace{0.3cm}
\includegraphics[width=0.18\textwidth, height=1.9cm]{rebuttal/imgs/cogvideox_5b_grid.pdf}
%\includegraphics[width=0.5\textwidth, height=3cm]{example-image-a}
\hspace{0.3cm}
\includegraphics[width=0.33\textwidth, height=1.9cm]{rebuttal/imgs/spec-comparison.pdf}
\vspace{-0.2cm}
\captionof{figure}{
\textbf{CogVideoX motion spectral volumes.}
We do the same analysis as in Fig. 3 and 4 of the main paper (zoom-in for details).
}
\label{fig:spec-analysis}

\vspace{-1em}
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{0.9}
\captionof{table}{\textbf{Additional baselines.} MotionCtrl and CameraCtrl for our original DiT base model; VD3D vs. AC3D for open-source CogVideoX.}
\label{table:metrics_camera_pose}
\begin{adjustbox}{width=1.0\textwidth}
\begin{tabular*}{1.0\textwidth}{@{\hspace{1pt}}l@{\extracolsep{\fill}}cccccccccc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{5}{c}{RealEstate10K} & \multicolumn{5}{c}{MSR-VTT} \\
\cmidrule(lr){2-6} \cmidrule(lr){7-11}
& \transerrorname & \roterrorname & \fidname & \fvdname & \clipscorename & \transerrorname & \roterrorname & \fidname & \fvdname & \clipscorename \\
\midrule
MotionCtrl (DiT) & 0.504 & 0.126 & 1.74 & 43.81 & 27.69 & 0.589 & 0.146 & 9.92 & 150.20 & 27.25 \\
CameraCtrl (DiT) & 0.513 & 0.138 & 1.62 & 42.10 & 27.73 & 0.566 & 0.143 & 8.15 & 146.77 & 27.51 \\
%VD3D (DiT) & 0.421 & 0.056 & 1.21 & 38.57 & \cellsecond{28.34} & \cellsecond{0.486} & \cellsecond{0.047} & \cellsecond{6.88} & \cellsecond{137.62} & \cellsecond{27.90} \\
\methodname (DiT) & \textbf{0.358} & \textbf{0.035} & \textbf{1.18} & \textbf{36.55} & \textbf{28.76} & \textbf{0.428} & \textbf{0.038} & \textbf{5.34} & \textbf{110.71} & \textbf{28.58} \\
\midrule
VD3D (CogVideoX) & 0.467 & 0.063 & 1.66 & 43.14 & 28.08 & 0.501 & 0.068 & 7.45 & 148.11 & 27.65 \\
\methodname (CogVideoX) & \textbf{0.374} & \textbf{0.039} & \textbf{1.27} & \textbf{38.20} & \textbf{28.62} & \textbf{0.431} & \textbf{0.039} & \textbf{5.52} & \textbf{116.04} & \textbf{28.38} \\
\bottomrule
\end{tabular*}
\end{adjustbox}
\vspace{-1.5em}

==> rebuttal/preamble.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}

\newcommand{\prob}{\mathbb{P}}
\newcommand{\Plucker}{Pl\"ucker\xspace}
\newcommand{\methodname}{AC3D\xspace}
\newcommand{\methodfullname}{Advanced 3D Camera Control}
\newcommand{\vdit}{VDiT\xspace}
\newcommand{\vditwithref}{\hyperref[sec:method:base-video-dit]{\vdit}\xspace}
\newcommand{\baselinename}{VDiT-CC\xspace}
\newcommand{\baselinewithref}{{\hyperref[sec:method:baseline-cc]{\baselinename\xspace}}}
\newcommand{\paramcount}{11.5B}
\newcommand{\ditxs}{\texttt{DiT-XS}}
\newcommand{\ditxl}{\texttt{DiT-XL}}
\newcommand{\camditxs}{\texttt{camera DiT-XS}}
\newcommand{\vidditxl}{\texttt{video DiT-XL}}
\newcommand{\linprobtrainspeedup}{15}
\newcommand{\retenkfull}{RealEstate10K\xspace}
\newcommand{\retenk}{RE10K\xspace}
\newcommand{\msrvtt}{MSR-VTT}
\newcommand{\Normal}{\mathcal{N}}
\newcommand{\StdNormal}{\Normal(0,\bm{I})}
\newcommand{\TruncNormal}[4]{\mathcal{TruncN}(#1, #2, #3, #4)}
\newcommand{\video}{\bm{x}}
\newcommand{\noise}{\bm{\varepsilon}}
\newcommand{\videonoised}{\tilde{\bm{x}}}
\newcommand{\videopred}{\hat{\bm{x}}}
\newcommand{\textcond}{\bm{y}}
\newcommand{\Vocab}{\mathcal{Y}}
\newcommand{\params}{\bm{\theta}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Rcfhw}{\R^{C \times F \times H \times W}}
\newcommand{\Rfhw}{\R^{F \times H \times W}}
\newcommand{\Denoiser}{D_{\params}}
\newcommand{\cin}{c_\text{in}}
\newcommand{\cout}{c_\text{out}}
\newcommand{\cskip}{c_\text{skip}}

\newcommand{\videotoken}{\bm{v}}
\newcommand{\cameracond}{\bm{c}}
\newcommand{\camextr}{\bm{C}}
\newcommand{\camintr}{\bm{K}}
\newcommand{\rotmat}{\bm{R}}
\newcommand{\transvec}{\bm{t}}
% \newcommand{\Plucker}{Plücker}
\newcommand{\pluckeremb}{\ddot{\bm{p}}}
\newcommand{\pluckertok}{\ddot{\bm{c}}}
\newcommand{\camdir}{\bm{d}} % camera direction
\newcommand{\latent}{\bm{z}} % RIN latents
\newcommand{\Loss}{\mathcal{L}} % RIN latents
% \newcommand{\read}{\textsf{read}} % read XAttn op
% \newcommand{\write}{\textsf{write}} % write XAttn op
\newcommand{\rinread}{\texttt{read}} % read XAttn op
\newcommand{\rinwrite}{\texttt{write}} % write XAttn op

% \newcommand{\TextSpace}{\mathcal{T}}
% \newcommand{\prompt}{\mathbb{c}}

% \newcommand{\ConfigA}{\textnormal{\textsf{Config A}}}
\newcommand{\config}[1]{{\mdseries\textsc{Config~\small\uppercase{#1}}}}

% Some cross-ref shortcuts
\newcommand{\refcfga}{\hyperref[sec:method:base-video-dit]{\config{a}}}
\newcommand{\refcfgb}{\hyperref[sec:method:base-video-dit]{\config{a}}}

\newcommand{\gqc}[1]{{\color{orange}[\textbf{Gordon:} #1]}}
\newcommand{\gq}[1]{{\color{orange}#1}}

\newcommand{\apprx}[1]{${\approx}{#1}$} % A better \approx command for regular text.


\newcommand{\cellbest}{\cellcolor{azure!35}}
\newcommand{\cellsecond}{\cellcolor{azure!10}}
\newcommand{\ours}{\textcolor{azure}{(ours)}}
\newcommand{\abl}[1]{\textit{#1}}

\newcommand{\transerrorname}{TransErr $\downarrow$}
\newcommand{\roterrorname}{RotErr $\downarrow$}
\newcommand{\fidname}{FID $\downarrow$}
\newcommand{\fvdname}{FVD $\downarrow$}
\newcommand{\clipscorename}{CLIP $\uparrow$}

\renewcommand{\paragraph}[1]{\vspace{.3em}\noindent\textbf{#1.}}

==> sec/1_intro_OLD.tex <==
\section{Introduction}
\label{sec:intro}

\input{figures/spec-analysis}
Foundational video diffusion models (VDMs), trained on internet-scale data, acquire abundant knowledge about the physical world~\cite{Sora}.
They learn not only the appearance and 2D dynamics, but also extensive 3D understanding~\cite{StableVideoDiffusion}.
However, most of this knowledge is stored implicitly and VDMs do not expose fine-grained control mechanisms over many desirable synthesis characteristics, like camera motion.
During the past year, we witnessed a surge of works that bring 3D camera control into foundational video models~\cite{MotionCtrl,CameraCtrl,DirectAVideo}, but the resulted camera following is not always precise, and the visual quality and scene motion are often compormised~\cite{VD3D}.
In this work, we analyze camera motion and its control in video diffusion models from first principles and develop several findings that allow us to incorporate precise 3D camera conditioning without degrading other aspects of the synthesis process.

Most modern text-to-video diffusion models (e.g., \cite{Sora,MovieGen,CogVideoX}) are built on top of a large-scale video latent diffusion transformer (\vdit)~\cite{LDM,DiT}, but are typically closed-source.
To analyze how \vdit s model camera motion, we train an \paramcount-parameters transformer on a dataset of 100M text/video pairs.
Then, we establish a simple camera control baseline model on top of it (which we name \baselinename) by adapting the VD3D~\cite{VD3D}'s pipeline.
We then analyze both \vdit\ and \baselinename\ to develop rigorous techniques that address imprecise control, visual quality degradation and reduced scene dynamics. 

First, we hypothesize that the motion induced by camera movements is a low-frequency type of motion, and as such, following the coarse-to-fine diffusion paradigm~\cite{PerspectivesOnDiffusion}, should emerge very early in the denoising process.
We analyze the motion spectral volumes~\cite{GID} of the generated videos with/without scene motion and with/without camera motion.
As observed from \cref{fig:spec-comparison}, camera motion indeed leads to increased low-frequency motion components, while the high-frequency ones remain similar to the videos with just scene motion.
Following this, we inspect motion spectra in different regions of the denoising process and find that the video diffusion creates the entire low-frequency camera motion in the first ${\approx}20$\% of the denoising process, which is depicted in ~\cref{fig:spec-analysis}.
This finding motivates us to revisit the typical camera conditioning schedule, where conditioning is applied at each step of the denoising process and where the camera control method is trained on the entire range of diffusion noise levels.
We find that applying camera conditioning in later regions of the denoising trajectory would only impair the scene motion, which is a higher frequency type of signal than camera motion.
Following this finding, we restrict both train and inference noise schedule to the first 40\% of the reverse diffusion process and observe that not only it increases training convergence \todo{\apprx{3.5}} times, but also improves visual quality \todo{X}\% and mitigates scene motion degradataion \todo{Y}\%.

Next, we investigate what vanilla video DiTs already know about the camera motion.
For this, we perform linear probing for camera trajectories on top \vdit\ internal representations, extracted from videos from RealEstate10k (RE10k)~\cite{RealEstate10k} (unseen by \vdit\ during training).
We observe that in the late \apprx{70}\% the denoising process, \vdit\ is implicitly performing accurate camera registration (see \cref{fig:linprob-analysis}).
Moreover, the camera information content peaks in the middle blocks, implying that it emerges in the early ones (to allow later layers use it to build subsequent visual features).
This guides us to apply camera conditioning in these first blocks to minimize the interference with other video representations.
That simple change allowed to reduce the amount of trainable parameters \apprx{4} times and accelerate training and inference by \apprx{\linprobtrainspeedup}\% without quality loss.

After that, we investigate the common distribution biases present in the existing datasets used for camera manipulation training.
First, we address the problem with RE10k, the dominant camera control training dataset, of being heavily biased towards static scenes.
We suspect that the model interprets camera conditioning as a cue to reduce scene dynamics, due to the conditioning ambiguity during training.
To mitigate this, we curate a subset of 20k in-the-wild videos with dynamic scenes, but static cameras (see \cref{fig:getty-static}) for which the camera conditioning branch can still be active to let the model disambiguate viewpoint conditioning from stillness.
Surprisingly, this simple data adjustment appears to be enough in mitigating RE10k distribution limitations and recovers most of the lost scene \todo{dynamism}, as we show in \todo{experiments section X}.

Besides, we observe that the camera trajectories, provided by RE10k \todo{(and other datasets?)} have arbitrary scaling, produced by COLMAP~\cite{colmap_sfm,colmap_mvs}.
This results in imprecise and inconvenient camera manipulation at test-time: when a user wants to, e.g. increase the length of the camera trajectory $2$ times, the model does not always align with this change, because it has learned to follow the camera conditioning only relatively.
To mitigate this, we develop a pipeline of rescaling camera extrinsics using an off-the-shelf metric depth estimator.
\todo{As our results in X show, this substantially improved camera following for our model.}

We \rephrase{accumulate} all these findings into a unified method, which we name \emph{\methodfullname} (\methodname).
Through ablation studies, we demonstrate the efficacy and importance of the developed techniques.
Finally, we compare it against state-of-the-art viewpoint manipulation approaches, including MotionCtrl~\cite{MotionCtrl}, CameraCtrl~\cite{CameraCtrl}, and VD3D~\cite{VD3D}: it shows up to \todo{X}\% better performance in terms of automatic evaluation metrics and \todo{Y}\% higher preferences in terms of user studies.

\input{figures/spec-comparison}


==> sec/3_method_OLD.tex <==
\section{Method}
\label{sec:method}

\input{figures/model-architecture}

We first describe our base video diffusion model and the baseline camera control method built on top of it~(\Cref{sec:method:baselines}).
\todo{Then, we proceed with the analysis of motion spectral volumes, linear probing and dataset biases, and how we use the insights to build rigorous and effective camera control.}

\subsection{Base models}
\label{sec:method:baselines}

\inlinesection{Base video diffusion transformer (\vdit).}
\label{sec:method:base-video-dit}
Following Sora~\cite{Sora}, most modern foundational video generators use the diffusion framework~\cite{DiffusionModels,DDPM} to train a large-scale transformer~\cite{Transformer} in the latent space of a variational autoencoder~\cite{VAE,LatentDiffusion,LDM} to generate videos from text descriptions.
We adopt the same design and, for a base video model, pre-train an \paramcount-parameters video DiT (VDiT) model~\cite{DiT} with 32-blocks of 4,096 hidden dimensionality for text-to-video generation in the latent space of CogVideoX~\cite{CogVideoX} $16$-channels $4{\times}8{\times}8$-compression autoencoder with the rectified flow diffusion parametrization~\cite{RecFlow}.
We use the T5~\cite{T5} encoder to produce text embeddings, which are passed into \vdit\ via cross-attention.
It was trained on a joint dataset of \apprx{100}M video/text pairs and \apprx{700}M image/text pairs of variable resolutions ranging from $17{\times} 144 {\times} 256$ to $121 {\times} 576{\times}1024$.
Such design is fairly standard and is followed by many existing works with little deviation (e.g., \cite{MovieGen,CogVideoX,LuminaT2X,OpenSora}), and we describe our particular architectural and training setups in detail in \cref{supp:model-details}.
\inlinesection{Baseline \vdit\ with Camera Control (\baselinename).}\label{sec:method:baseline-cc}
For a baseline camera control method, we implement a simple ControlNet-like~\cite{ControlNet} pipeline on top of our \vdit.
Following the most works (e.g., \cite{MotionCtrl, CameraCtrl}), we use the RealEstate10k~\cite{RealEstate10k} dataset of \todo{60k} (text, video, camera trajectory) triplets ${(\video_i, \textcond_i, \cameracond_i)}_{i=1}^N$ and train a new set of model parameters to input the camera information into the model.
Camera trajectories $\cameracond \in \R^{f\times25}$ are provided in the form of camera extrinsics $\camextr_f \in \R^{4\times 4}$ and intrinsics $\camintr_f \in \R^{3\times 3}$ for each $f$-th frame $\video_f$.

For the conditioning mechanism, we adapt VD3D~\cite{VD3D} since it is most similar to our transformer-based pipeline, while other methods are built on top of UNet-based~\cite{U-net} backbones.
Specifically, we use Plücker camera representations, which are projected to the same dimensionality and, to account for latent autoencoder downsampling, resolution as the video tokens via a fully-convolutional encoder to produce camera tokens.
Next, we instantiate a sequence of lightweight DiT blocks with 128 hidden dimensionality and 4 attention heads each.
To mix the camera information into video representations, we found a simple summation to be sufficient, which we perform before each main DiT block.
Besides, we found it useful to perform cross-attention from video tokens to camera tokens as a form of feedback connection~\cite{ControlNet++}.
We illustrate our baseline architecture \baselinename in \cref{fig:architecture} and elaborate on it in \cref{supp:model-details}.

We train the new parameters (with the \vdit backbone being frozen) with the rectified flow objective~\cite{RecFlow} and logit-normal noise distribution~\cite{EDM,SD3}.
Similar to prior works (e.g., \cite{VD3D, 4DiM}), we apply a 10\% camera dropout to support classifier-free guidance (CFG)~\cite{CFG} later.
Notably, we train \baselinename\ only at the $256^2$ resolution: since camera motion is a low-frequency type of signal (which is fully unveiled at lower resolutions), and the main \vdit backbone is frozen, we found that such design generalizes to higher resolutions out-of-the-box.
% During inference, at each time step, we input text prompts with the CFG weight of 8.0 and camera embeddings with CFG weight of 3.0.
During inference, at each time step, we input text prompts and camera embeddings with the CFG weight of 8.0.
\todo{We use various CFGs, right?}

We observe that this baseline model, being built on top of our powerful \vdit, already achieves good overall quality and camera control.
However, it still struggles with degraded visual quality, reduced scene motion, and sometimes imprecise camera following.
To improve the design, we analyze our \vdit\ backbone to understand how camera motion is modeled and represented by it, and then inspect \baselinename's failure cases and where they arise to rigorously address them.

\subsection{How camera motion is modeled by diffusion?}
\label{sec:method:motion}

We start by analyzing how camera motion is modeled by a pre-trained video diffusion model (i.e., before camera control is incorporated).
We hypothesize that the motion induced by camera transitions is a low-frequency type of signal (unless it's unnatural and undesirable shaky camera movements) and investigate the motion spectral volumes of the generated videos at different steps of the denoising trajectory.

For this, we generate 200 in-the-wild videos with our \vditwithref\ model with 80-steps denoising trajectory and manually annotate them into 4 categories: videos with only scene motion, videos with only camera motion, videos with both scene and camera motion, and others (see \cref{supp:motion-analysis-details} for details).
During generation, we save the denoised predictions at each denoising step.
After that, following \cite{GID}, we estimate the optical flow and compute motion spectral volumes for each generated video at each step.
We visualize these lines with 95\% confidence intervals in \cref{fig:spec-comparison}: videos with camera motion exhibit higher amplitudes than scene-motion-only videos for low-frequency components while having similar characteristics for high-frequency ones.
This supports the conjecture that the camera motion is a low-frequency type of signal.
We also depict an example of a generated video with both scene and camera motion with 4 denoising steps on \cref{fig:spec-analysis:visual-example}: one can observe that the camera movement has been fully produced by $t=0.9$ (first 10\% of the rectified flow denoising process), while scene motion details like hand movements of the subjects is not finalized even till $t=0.5$.

Inspired by this finding, we pose the question: when does exactly a video diffusion model determine the camera?
To answer it, we plot aggregated spectral volumes for different timesteps on \cref{fig:spec-analysis:spec-per-timestep} and also their ratio with respect to the last timestep $t=0$ (for which all the motion has been produced), and inspect when different types of motion kick in during the denoising process.
\cref{fig:spec-analysis:spec-per-timestep} (right) shows that the low-frequency motion components fill up to \apprx{84}\% at $t=0.9$ (the first 10\% of the denoising process), while high frequency ones are not well complete even till $t=0.6$.

An immediate consequence of this observation is that trying to control the camera later in the denoising trajectory is unnecessary and will not influence the manipulation result.
But surprisingly, we observe that not only it is unnecessary but also detrimental to the scene motion and overall visual quality.
Following this insight, we restrict both our train-time noise levels and test-time camera conditioning schedules to only cover the first 40\% of the reverse diffusion trajectory.
As tables and figures~\todo{refs?} show, it improves the convergence speed by \todo{X}, motion quality by \todo{Y}, camera following by \todo{Z}.

\subsection{What video DiT knows about camera motion?}
\label{sec:method:linprob}

\label{sec:method:knowledge}
\input{figures/linprob-analysis}

Foundational video models acquire rich knowledge about the physical world, and we hypothesize that they store information about the camera signal within their representations.
To investigate this, we perform linear probing of our base \vditwithref\ model on the RealEstate10k~\cite{RealEstate10k} dataset (unseen during training) for camera extrinsics.

Specifically, we take 1,000 random 49-frame videos from RealEstate10k, feed them into \vdit\ under 8 noise levels $(1/8, 2/8, ..., 1)$, and extract the activations for all 32 DiT blocks.
Next, we split them into 900 train and 100 test videos and train a ridge linear regression model to predict the rotation pitch/yaw/roll angles and translation vectors for the entire viewpoint trajectory ($49\times 6$ target values in total).
This results into $8 \times 32$ trained models and we report the rotation and (normalized) translation errors on a held-out test set of 100 videos in \cref{fig:linprob-analysis}.

Surprisingly, \vdit can predict the camera signal very accurately, achieving minimum test errors of \apprx{0.025} and \apprx{0.48} for rotation and translation prediction, respectively.
The knowledge quality starts increasing around the layer \#9 and peaks in the range of \#13-21.
We reason that since the camera information in block \#13 is stored in such a disentangled manner, then the model is using it to build other representations, and conditioning the camera at this point is both risky and unnecessary and would interfere with other visual features.
In this way, we propose to input the camera only in the first \#8 blocks and leave the rest 24 DiT blocks unconditioned.
What we found empirically in \cref{SecExp} is that this didn't decrease the performance of our method, while reducing the amount of trainable parameters \apprx{4} times and training speed \apprx{\linprobtrainspeedup}\%.

\subsection{Mitigating training data limitations}
\label{sec:method:data}

\inlinesection{Data Distribution}.\label{sec:method:data:getty-static}
Estimating camera parameters from internet videos remains challenging, as leading methods like~\cite{particlesfm, colmap_mvs, colmap_sfm, dust3r} frequently fail when processing videos containing dynamic scene content.
This limitation has resulted in camera-annotated datasets being heavily biased toward static scenes, particularly evident in \retenkfull\ (\retenk)~\cite{RealEstate10k}, which is the predominant dataset for training camera-controlled video generation models~\cite{MotionCtrl,CameraCtrl,VD3D}.
We hypothesize that models fine-tuned on such data interpret camera position information as a signal to suppress scene dynamics.
This bias persists even when jointly training on unconstrained 2D video data~\cite{4DiM}, because the camera conditioning branch is only activated when camera parameters are available, which occurs exclusively for static scenes from \retenk, as static scenes remain the only reliable source for accurate camera annotation.
To address this fundamental limitation, we propose an alternative approach: rather than attempting to annotate dynamic scenes (which proved unsuccessful in our extensive preliminary research, even with state-of-the-art methods~\cite{dust3r}), we curate a collection of 20k in-the-wild videos featuring dynamic scenes captured by stationary cameras (see \cref{fig:getty-static}).
With stationary cameras, the camera position is inherently known (we can assign fixed arbitrary extrinsics), allowing us to maintain active camera conditioning during training.
This approach enables the camera conditioning branch to remain active during training while exposing the model to dynamic content, helping it distinguish between viewpoint conditioning and scene stillness.
Our experiments in Sec.~\ref{sec:experiments} demonstrate that this straightforward yet effective data curation strategy successfully mitigates the distributional limitations of \retenk, restoring much of the lost scene \todo{dynamism} while maintaining precise camera control.

\inlinesection{Scaling Bias}.
Classical feature-based camera estimation~\cite{colmap_sfm, colmap_mvs} outputs camera trajectories with arbitrary scale, as it does not possess any priors about the absolute size of objects in the scene. For example, a house might appear identical to a small object like an apple when viewed from the appropriate distance, making it impossible to determine absolute scale from visual features alone. This lack of scale awareness complicates precise user control over camera trajectories: while the model can determine the camera's direction, it remains unaware of the magnitude of each movement, as demonstrated in \cref{sec:experiments:scale-ablations}.
Ideally, all camera trajectories should be aligned to a consistent reference scale.
A natural reference would be a metric scale, now achievable due to recent advances in metric depth estimation \cite{Metric3D}.
We propose a method to rescale camera trajectories across all data using the following steps:
\begin{enumerate}
\item Obtain 3D points from the COLMAP output and render the COLMAP depth $D^f_c$ from these points for each frame.
\item Estimate the metric depth $D^f_m$ for each frame using a pre-trained zero-shot metric depth estimator~\cite{Metric3D}.
\item Calculate the re-scaling parameter $\hat{\lambda}$ by solving the optimization problem $\hat{\lambda} = \arg\min_\lambda \mathbb{E}_{f \sim F} \left| \lambda D^f_c - D^f_m \right|$, where $F$ is the total number of frames.
\item Set the camera translation vector $\hat{\bm{t}}_c$ to $\hat{\lambda} \bm{t}_c$.
\end{enumerate}
In Sec.~\ref{sec:}, we show that this approach provides significantly improved control over the magnitude of the camera movements.

\input{figures/getty-static}

\subsection{Miscellaneous improvements}
\label{sec:method:misc}
In addition to our core analysis, we introduce several auxiliary techniques that enhance model performance.

\inlinesection{1D temporal camera encoder.}
\label{sec:method:misc:high-res-enc}
\baselinewithref\ processes video in the autoencoder's latent space with $4\times$ temporal compression~\cite{CogVideoX}, raising the question of how to incorporate full-resolution camera parameters.
While camera poses could be naively downsized (e.g., subsampled or reshaped) to match the latent resolution, this would force small \ditxs\ blocks to process compressed camera information.
Instead, we implement a sequence of causal 1D convolutions that transform a $F \times 6$ sequence of \Plucker\ coordinates for each pixel into a $(F // 4) \times 32$ representation (see \cref{supp:model-details}).
This architecture improves \todo{X} by \todo{Y} compared to simple downsampling.

\inlinesection{Separate text and camera guidance.}
\label{sec:method:misc:separate-cfg}
Text and camera signals require different guidance weights due to their distinct nature, motivating us to separate their classifier-free guidance (CFG).
We formulate the guidance equation as:
\begin{equation}\label{eq:separate-cfg}
\hat{s}(\bm x | \textcond, \cameracond) = (1 + w_y + w_c) s_\theta(\video | \textcond, \cameracond) - w_y s_\theta(\video | \cameracond) - w_c s_\theta(\video | \textcond),
\end{equation}
where $\hat{s}(.)$ denotes the final update direction used during synthesis, $s_\theta$ represents the model's predicted update direction, $\textcond$ and $\cameracond$ are text and camera conditions, and $w_y$ and $w_c$ are their respective CFG weights.

\inlinesection{ControlNet with feedback.}
\label{sec:method:misc:controlnet++}
Traditional ControlNet~\cite{ControlNet}, used in recent camera control methods~\cite{MotionCtrl,CameraCtrl,VD3D}, only processes conditioning signals without accessing the main branch.
Our experiments show that adding cross-attention from video tokens to camera tokens in transformer computations enables better camera representations.
This modification behaves as a feedback mechanism~\cite{ControlNet++} provided by the main synthesis branch to the camera processing branch.


==> tables/camera_poses_old.tex <==
\newcommand{\transerrorname}{TransErr $\downarrow$}
\newcommand{\roterrorname}{RotErr $\downarrow$}
\newcommand{\fidname}{FID $\downarrow$}
\newcommand{\fvdname}{FVD $\downarrow$}
\newcommand{\clipscorename}{CLIP $\uparrow$}

\begin{table*}[!t]
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{0.9}
\caption{\textbf{Camera pose evaluation.} We evaluate all the models using reference camera trajectories from the RealEstate10K~\cite{RealEstate10k} test set. We compute translation and rotation errors based on the estimated camera poses from generations using ParticleSfM \citep{particlesfm}. Ablations (lower part) are described in \cref{sec:experiments:ablations}.}
\label{table:metrics_camera_pose}
\begin{adjustbox}{width=\textwidth}
\begin{tabular*}{1.0\textwidth}{@{\hspace{1pt}}l@{\extracolsep{\fill}}cccccccccc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{5}{c}{RealEstate10K~\cite{RealEstate10k}} & \multicolumn{5}{c}{MSR-VTT~\cite{MSRVTT}} \\
\cmidrule(lr){2-6} \cmidrule(lr){7-11}
& \transerrorname & \roterrorname & \fidname & \fvdname & \clipscorename & \transerrorname & \roterrorname & \fidname & \fvdname & \clipscorename \\
\midrule
MotionCtrl~\cite{MotionCtrl} & 0.477 & 0.094 & 2.99 & 61.70 & 26.46 & 0.593 & 0.137 & 16.85 & 283.12 & 24.11 \\
CameraCtrl~\cite{CameraCtrl} & 0.465 & 0.089 & 2.48 & 55.64 & 26.81 & 0.587 & 0.132 & 12.33 & 201.33 & 25.05 \\
VD3D (FIT)~\cite{VD3D} & \cellsecond{0.409} & \cellsecond{0.043} & \cellsecond{1.40} & \cellsecond{42.43} & 28.07 & 0.504 & 0.050 & 7.80 & 165.18 & 26.89 \\
VD3D (DiT) & 0.421 & 0.056 & 1.21 & 38.57 & \cellsecond{28.34} & \cellsecond{0.486} & \cellsecond{0.047} & \cellsecond{6.88} & \cellsecond{137.62} & \cellsecond{27.90} \\
\methodname~\ours & \cellbest{0.358} & \cellbest{0.035} & \cellbest{1.18} & \cellbest{36.55} & \cellbest{28.76} & \cellbest{0.428} & \cellbest{0.038} & \cellbest{5.34} & \cellbest{110.71} & \cellbest{28.58} \\
\midrule
w/o camera cond & 0.591 & 0.188 & 5.20 & 90.38 & 27.13 & 0.694 & 0.195 & 4.86 & 102.18 & 28.93 \\
w/o noise scheduling & 0.451 & 0.050 & 1.20 & 38.33 & 28.44 & 0.566 & 0.071 & 5.93 & 127.63 & 28.04 \\
w/o truncated noise sampling & 0.378 & 0.032 & 1.24 & 38.24 & 28.56 & 0.444 & 0.043 & 6.10 & 117.34 & 28.40 \\
w/o camera cfg & 0.372 & 0.039 & 1.67 & 41.12 & 28.22 & 0.453 & 0.041 & 5.37 & 112.13 & 28.31 \\
w/o static camera dropout & 0.353 & 0.031 & 1.12 & 36.77 & 28.56 & 0.432 & 0.037 & 6.23 & 115.11 & 28.03 \\
w/o metric scaled data & 0.371 & 0.040 & 1.35 & 41.20 & 28.76 & 0.451 & 0.040 & 5.33 & 110.71 & 28.46 \\
w/o dropping camera context & 0.371 & 0.036 & 1.22 & 39.01 & 28.11 & 0.457 & 0.041 & 6.59 & 118.12 & 28.22 \\
w/o limiting camera cond to 8 blocks & 0.357 & 0.036 & 1.27 & 37.11 & 28.74 & 0.431 & 0.038 & 5.66 & 119.94 & 28.25 \\
with 2D training & 0.487 & 0.103 & 3.78 & 70.40 & 27.59 & 0.556 & 0.131 & 5.08 & 106.88 & 28.79 \\
\bottomrule
\end{tabular*}
\end{adjustbox}
\end{table*}

